MOHAQ: Multi-Objective Hardware-Aware Quantization of Recurrent Neural Networks

The compression of deep learning models is of fundamental importance in deploying such models to edge devices. The selection of compression parameters can be automated to meet changes in the hardware platform and application using optimization algorithms. This article introduces a Multi-Objective Hardware-Aware Quantization (MOHAQ) method, which considers hardware efficiency and inference error as objectives for mixed-precision quantization. The proposed method feasibly evaluates candidate solutions in a large search space by relying on two steps. First, post-training quantization is applied for fast solution evaluation (inference-only search). Second, we propose the "beacon-based search" to retrain selected solutions only and use them as beacons to know the effect of retraining on other solutions. We use a speech recognition model based on Simple Recurrent Unit (SRU) using the TIMIT dataset and apply our method to run on SiLago and Bitfusion platforms. We provide experimental evaluations showing that SRU can be compressed up to 8x by post-training quantization without any significant error increase. On SiLago, we found solutions that achieve 97\% and 86\% of the maximum possible speedup and energy saving, with a minor increase in error. On Bitfusion, beacon-based search reduced the error gain of inference-only search by up to 4.9 percentage points.

==> files/bio.tex <==
 \vskip -2\baselineskip plus -1fil 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/nesma1.jpeg}}]{Nesma M. Rezk}received her bachelor and masters degrees in computer and systems engineering from the faculty of engineering, Ain Shams University, Egypt in 2010 and 2015, respectively. 

From 2011 to 2016 she was a teaching and research assistant in the faculty of engineering, Ain Shams University. Since 2016, she has been a PhD student in the School of Information Technology at Halmstad University, Sweden. Her research interests include embedded systems, deep learning applications, and design of domain-specific architectures.  
\end{IEEEbiography}
 \vskip -3\baselineskip plus -1fil 

\begin{IEEEbiography}[{\includegraphics[width=1.25in,height=1.25in,clip,keepaspectratio]{images/tomas.png}}]{Tomas Nordström} received the M.S.E.E. degree in 1988 and a Ph.D. degree in 1995, both from Luleå University of Technology, Sweden. Between 1996 and 1999, he was with Telia Research, where he developed broadband Internet communication over twisted copper pairs. In December 1999, he joined the FTW Telecommunications Research Center Vienna, Austria, working as a researcher in the field of broadband wireline access.
In 2012 he became full Professor in Computer Engineering at Halmstad University, Sweden,  in the area of energy-efficient embedded computers; and since 2019, he is full Professor in Embedded and Intelligent Systems at Umeå University, where his research is focusing on edge computing, intelligent IoT systems, and embedded machine learning.


\end{IEEEbiography}
 \vskip -3\baselineskip plus -1fil 
\begin{IEEEbiography}[{\includegraphics[width=1.25in,height=1.25in,clip,keepaspectratio]{images/dimit.png}}]{Dimitrios Stathis} received his Diploma in Electr. \& Comp. Engineering and a M.Sc. in Microelectronics and Computer Systems, both from the Democritus University of Thrace, Xanthi, Greece in 2013 and 2016 respectively. He received his second M.Sc. degree in Embedded Systems from KTH, Stockholm, Sweden in 2017. He is currently working towards the Ph.D. degree at the KTH, Stockholm, Sweden. His research interests include Computer Architectures and ASIC design for multimedia applications and Artificial Neural Networks.
\end{IEEEbiography}
 \vskip -3\baselineskip plus -1fil 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{images/zain.jpg}}]{ Zain-ul-Abdin} completed his PhD degree in Computer Science from Örebro University in 2011 and until recently held an appointment as Associate Professor at Halmstad University. 

He has played a key role in a number of research projects such as Smart Multicore Embedded Systems (SMECY), High-Performance Embedded Computing (HiPEC), and Towards Next Generation Embedded Systems (NGES). In these projects he has worked in close collaboration with
% ToNo suggestion:
European industrial and academic partners.
%the Swedish Defence Research Agency (FOI) and industrial partners such as ST- Microelectronics, Ericsson, Adapteva, and Saab. 
% ToNo editing:
He has authored more than 42 journal and conference articles;  bin active as TPC for several leading conferences; and has served as an external reviewer for multiple journals (e.g. IEEE-TSP and IEEE-Micro).
% He has authored more than 42 journal and conference articles and has been awarded the best paper prize in the PhD forum of 19th Field-programmable Logic and Applications conference (FPL’09). He has sat on the technical program committee of several leading conferences and has served as an external reviewer for journals (IJRC, IEEE-TSP, IEEE-Micro, JSP).
\end{IEEEbiography}
 \vskip -2\baselineskip plus -1fil 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{images/eren.jpg}}]{Eren Aksoy}
 is an Associate Professor (Docent) at Halmstad University in Sweden. He obtained his Ph.D. degree in computer science from the University of Göttingen, Germany, in 2012. After his PhD, he spent 3 years as a postdoctoral research fellow at the Karlsruhe Institute of Technology in the H2T group. He has been a visiting scholar at Volvo GTT and Zenseact AB in Sweden, working on AI-based perception algorithms for autonomous vehicles. He serves as an Associate Editor in different high-ranking journals and conferences (RA-L, IROS, Humanoids, etc.). His research interests include action semantics, computer vision, AI, and cognitive robotics. He has been working on creating the semantic representation of visual experiences to achieve a better environment and action understanding for autonomous systems such as robots and unmanned vehicles. 

\end{IEEEbiography}
 \vskip -3\baselineskip plus -1fil 
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{images/AH.jpg}}]{Ahmed Hemani }
 did his doctorate from KTH in 1993. His doctoral thesis work on HLS was commercialized by CADENCE as Visual Architect and was the first HLS product from CADENCE. He also pioneered the concept of Networks on Chip that is now a major research area and widely adopted by the computer architecture community. Later he contributed to Globally Asynchronous and Locally Synchronous Clocking. His most recent contribution has been Synchoros VLSI design that is the basis for Silicon Lego (SiLago) design framework. He has also worked widely in industry at National Semiconductors, ABB, Ericsson, Philips Semiconductors and NewLogic. He was also part of three start-ups. His current research interests are in synchoros VLSI design as the basis for automating application and system level synthesis of ASIC like efficient hardware. 
 %ToNo removed
 % He is also pursuing in-situ memristor based computation and applying it to neuromorphic computation.
\end{IEEEbiography}
% \EOD

==> files/method.tex <==
\label{sec:method}
This section discusses the details of our proposed method for the Multi-Objective Hardware-Aware Quantization (MOHAQ) of the SRU-model for speech recognition. First, we explain how we apply the post-training quantization on the SRU. Then, we present the optimization algorithm used to select the layers' precisions guided by the hardware model. Finally, we explain how to enable retraining in a multi-objective search for setting mixed precision quantization configurations.
\subsection{Post-training quantization of SRU model}
The Simple Recurrent Unit (SRU) was initially designed to overcome the parallelization difficulty in LSTM and other recurrent units. Outputs from the previous time-steps are used in the current time-step operations. This property makes it impossible to fully parallelize the M$\times$V operations over multiple time steps. In SRU, the outputs from the previous time-step are excluded from M$\times$V computations and only used in element-wise computations.

Another side effect for excluding the recurrent inputs from M$\times$V operations is that the number of weights used in the recurrent operations decreases significantly. Thus, it becomes possible to also exclude the recurrent part from low-precision quantization. We apply low-precision quantization on weights and activations used in M$\times$V operations only. Other weights are kept in a 16-bit fixed-point format. By doing so, We achieve our goal of reducing the model's overall size while keeping it performing with a low error rate. % Excluding the bias from quantization of LSTM has been done without significant effect on the model size~\cite{quantize-aji2020}.
%The last sentence here is somehow not linked to the context!-- Eren
We have both 16-bit fixed-point and integer precisions in the same model in different layers in our work.  We here explain how quantization has been applied to the weights and activations during inference and how we move from fixed-point to integer operations and the reverse.
\begin{itemize}
\item \textbf{Weights integer quantization with clipping:}
We applied integer linear quantization on the weight matrices. We used the Minimum Mean Square Error (MMSE) method to determine the clipping threshold~\cite{Sung_MMSE_2015}. We used the implementation for CNN quantization provided by OCS paper on github~\cite{postq-ocs-zhao19} as a base for our implementations. We then modified the implementation to work with SRU units and to support varying precision per layer. The range of the quantized values are [-128:127], [-8:7], and [-2:1] for 8-bit, 4-bit, and 2-bit, respectively.
\item \textbf{Weights 16-bit fixed-point quantization:}
It is used for the recurrent weights, bias vectors, and weight matrices that might be chosen to have 16-bit. Depending on the range of data, we compute the minimum number of bits required for the integer part. The rest of the 16-bits are used as a sign bit and the approximated fraction part.
\item \textbf{Activation integer quantization with clipping:}
Integer quantization of activations is similar to weights. However, since we cannot compute the range of vectors required for clipping threshold computation, we calculate the expected ranges. To compute expected ranges, we first use a portion of the validation data sequences. The predicted range of a given vector is calculated as the median value of the ranges recorded while running the validation sequences. In our experiments, 70 sequences were enough to compute the expected ranges. 
\item \textbf{Activation re-quantization to 16-bit fixed-point:}
The activations are quantized to 16- bits the same way as the weights. In the case of having a vector that is an output of integer operation, we found it necessary to re-quantize the values into fixed-points by dividing them by a scale value. The scale value is computed to return the vector range to the same range if quantization was not applied. The range of Non-quantized data is computed using a portion of the validation data sequences while using original model weights and activation, a.k.a, turning off quantization.
\end {itemize}

\subsection{Multi-objective quantization of neural network models}
\label{sec:method-inference}
During the compression/quantization of NN models, we have two types of objectives. The first one is the model performance metric such as the accuracy or the error. The second type of objective is related to the efficiency of the hardware platform, such as memory size, latency, energy consumption, and area. Treating the problem as a multi-objective problem provides the designer with various solutions with different options. The embedded system designer then can decide which solution is a trade-off suitable for the running application. We have used a Genetic Algorithm (GA) as it is one of the efficient multi-objective search optimizers. The multi-objective GA we used is called NSGA-II provided by the Pymoo python library~\cite{NSGA2-Deb-2002,pymoo}.
Most of the automated hardware-aware compression/quantization work uses a single objective and provides a single answer. The reason is that many compression methods require training or retraining to compensate for the accuracy loss caused by compression. The selection of the compression/quantization configuration is made iteratively during training epochs. Trying to turn the problem into a multi-objective problem would make it necessary to retrain all the evaluated solutions in the search space, and that would be infeasible. Our approach to tackle this problem relies on two observations. The first is that researchers are progressively enhancing post-training compression/quantization techniques. Thus, it is possible to evaluate candidate solutions by running inference only without any retraining. That is also useful for the case when the training data is not available. The second observation is that a retrained model using one candidate solution variables can be used as a retrained model for neighbor candidate solutions in the search space. We use this observation  in a method we call \textit{"beacon-based search"} (more explained in Section~\ref{sec:beacon}). So, if the inference-only search failed to find accuracy-wise accepted solutions, the beacon-based search can be applied. Nevertheless, if the designer wants, the beacon-based search can be applied from the beginning. The complete search framework is demonstrated in Figure~\ref{fig:idea}.
\begin{figure}[h]
   \centering
   \includegraphics[width=0.6\columnwidth]{images/idea.png}
    \caption{Steps of the Multi-Objective Hardware-Aware Quantization (MOHAQ) method. The designer inputs the model pre-trained parameters, the hardware platform objectives equations, and any hardware constraints if they exist. Then the designer can apply inference-only search or beacon-based search. The beacon-based search is the search method that requires retraining of the model using some candidate solutions variables. The output of the search is a Pareto set of optimal solutions. Suppose the inference-only search resulted in solutions that had unaccepted accuracy levels. In that case, the designer can repeat the search using the beacon-based method.}
    \label{fig:idea}
\end{figure}

Our problem is to select the precision for weights and activations per layer. A candidate solution has a number of variables that equals twice the number of layers. That is because each layer requires precision for the weight and precision for the activation. The possible precisions covered in this work are 2, 4, 8 bits integer, and 16-bit fixed point. We skipped precisions like 3, 5, and 6 because they are not frequently found in hardware platforms. However, the method is generic, and other precisions can be included. The candidate solutions variables are encoded into genetic algorithm representation. We use discrete values for the solutions variables that are 1, 2, 3, and 4. 2- bit is encoded into 1, 4-bit is encoded into 2, 8-bit is encoded into 3, and 16-bit is encoded into 4. 
In addition to encoding and decoding, we select the number of generations, define fitness functions and constraints, then keep the library default configuration for the rest of GA steps such as the crossover, mutation, and selection. For each objective, we define a fitness function. All the objectives have to be either minimization or maximization objectives. Since Pymoo by default treats objectives as minimization objectives, we change the maximization objectives to be minimization objectives by negating them. %One candidate solution is composed of the precision of each layer and activation.
%In our model we have 4 layers with 3 projection layers and one fully connected layer. Thus, we have 8 weights and 8 activations in each solution. Each value in the solution can either be 2, 4, 8 , or 16. Where, 2, 4, 8 are for integer quantization and 16 is for fixed point quantization. These values cannot be used directly in the GA. Encoding the values is a necessary step in GAs.


Initially, the search relies on post-training quantization (inference-only search). The evaluation of candidate solutions does not incorporate any training, and thus it is possible to carry out the search within a reasonable time. To evaluate one solution error objective, we run the inference of the model and get the inference error value as the error objective that we want to minimize.
One issue related to our problem is which data set we are going to use during this evaluation. The testing set cannot be used for this purpose, and an extra set that has not been seen before by the model would be the best fit. However, we do not have that set. Thus, we will instead use the validation set. The validation set has been used during training, and the model has some information about it. In our experiments, we have noticed that the gap between the validation error and the testing error varies along with a wide range. We experimented with splitting the validation data into four splits, running inference four times using the four splits separately, and then taking the maximum error to better correspond to the testing error. This better corresponding is an interesting effect, and we plan to explore it in our future experiments further. 
Luckily, it is possible to distribute the algorithm for speedup if required in a simple way. In our case, the evaluation of solutions is the most time-consuming part. Since the evaluations of candidate solutions in one generation are not related, they can be distributed on multiple GPUs~\cite{Rezk-distGA-2014}.


\subsection{Beacon-based Search (Retraining-based Multi-objective Quantization) }
\label{sec:beacon}
In this work, we have been using post-training quantization as a fast quantization method to speedup the evaluation of candidate solutions during the search for optimum quantization configuration. However, at high compression ratios, post-training quantization may not guarantee acceptable accuracy levels. In this case, no escape from applying retraining. But again, it is not feasible to retrain all evaluated solutions during the search. Therefore, we need to find a method that can attain retraining benefits without retraining all solutions. Literature has shown that quantization to 16-bit or 8-bit mostly does not cause any accuracy loss. While lower precisions like 6, 5, and 4-bit would require efficient post-training quantization techniques such as clipping to minimize the accuracy loss. And then, compressing the model more would require retraining the model using the new precision. Imagining that the baseline pretrained model is the base source of the NN model information, decreasing the precision more and more resembles going far and far away from the source and losing more important information. In this case, we need a rectifier, an amplifier, or a beacon to make the source information clear again for far solutions.


\begin{figure}[h]
   \centering
   \includegraphics[width=0.4\columnwidth]{images/beacons.png}
    \caption{An illustration for the beacon-based search idea. The red circle is the search space. The yellow circles are areas where post-training quantization can be applied with accepted accuracy loss. The first yellow circle at the left surrounds the baseline model. Beacons (retrained model using low precision configurations) are placed in other areas to allow post-training quantization with accepted accuracy loss.  }
    \label{fig:beacons}
\end{figure}
The idea of the beacon-based search (visualized in Figure~\ref{fig:beacons}) claims that solutions that cannot successfully apply post-training quantization on the pre-trained model need another model's parameters that are more suitable for them to use. These parameters (beacon parameters) can be generated by retraining the baseline model using a low precision configuration similar to those solutions. Her-by, we define a neighborhood of solutions as an area in the search space around a beacon where post-training quantization can be applied to solutions in this area using the beacon parameters with a similar retraining effect on the accuracy. We know that one solution composes of the precisions of weights and activations of model layers. Thus, neighbor solutions are solutions that the differences between their precisions are less than a given threshold. The validity of this concept is examined by an experiment. We have generated some beacons by retraining the model using low precision solutions variables.

\begin{figure}[h]
   \centering
   \includegraphics[width=0.6\columnwidth]{images/beacon_2.png}
    \caption{A plot for the error enhancement using one retrained model parameters (beacon). Each point corresponds to a neighbor solution to the retrained model solution. The x-axis corresponds to the increase in the baseline model error by evaluating solutions using baseline model parameters. The y-axis corresponds to the error degradation using the retrained parameters.}
    \label{fig:beacon_2}
\end{figure}

Then, for all solutions during the search, we found solutions that are neighbors to those beacons, and we evaluated the solutions using post-training quantization twice. Once using the baseline pre-trained model parameters and once using the neighbor beacon parameters. In Figure~\ref{fig:beacon_2}, we show a plot for an example of these beacons. We have similar plots for more beacons, but we cannot show all of them to save space. Each point in the plot is a solution that is neighbor to the beacon. The x-axis shows the increase in the error reached by solution when evaluated using the baseline model parameters compared to baseline error. The y-axis shows the decrease in the error value when the beacon parameters have been used for evaluating the same solution using post-training quantization. To understand how this plot is generated by an example, we show the computation for one point (solution). The baseline model error rate is 17.2\% and applying post-training quantization on this solution using the baseline model parameters gives an error rate of 25.2\%. Applying post-training quantization on the same solution using the beacon parameters gives 20\%. Thus, to add this solution to the plot, we put 8 ($25.2-17.2$) on the x-axis and 5.2 ($25.2-20$) on the y-axis.       

In Figure~\ref{fig:beacon_2}, we see that almost all the points follow the same relation between the increase in the error using baseline model parameters and the decrease in the error using the beacon parameters. This relative monotonic behavior clarifies that there is no need to retrain the model for all evaluated solutions during the search. We only need to retrain the model for one solution in some areas in the search space. To retrain the model, we used the same approach used in Binary-connect~\cite{lowp-binary-connect}. Quantized weights are used during the forward and backward propagation only, while full
precision weights are used for the parameters update step. Therefore, in the retrained model, we always have the floating-point parameters, which can be used as a basis for other quantization configurations.
The term beacon is also used during the swarm robots search. When the simple robots do not have enough sensors for efficient communication, some robots are turned into beacons and stand still to guide others~\cite{swarm-beacons-2013}. Similarly, when our search reaches an area with no beacons, one solution is turned into a beacon by retraining the model using this solution variables. By the end, we get a solution set that considered the retraining effect on candidate solutions. Later on, when the designer selects a solution from the Pareto optimal set, the designer can use the beacon parameters directly or retrain the model using the selected solution parameters. 



%That for a given solution that cannot apply post-trining  
%Retraining is a time consuming task. If we need retrain the model per each solution evaluation, this will be very time consuming especially for large models. 
%If we want to apply multi-objective search on compression/quantization of neural network while retraining is enabled, it will not be a straightforward task. That is because we cannot retrain each solution within its evaluation during the search. In this section, we explain how to overcome this problem in the case of quantization. 
% We have selected some solutions, retrained them, and then used the retrained parameters for evaluating neighbor solutions. The degradation in the error we get by retraining a model using a specific solution parameter is similar to the degradation we get when using these parameters to evaluate neighbor solutions. 
%Figures~\ref{fig:beacon_1} and~\ref{fig:beacon_2} show the effect of using two different retrained models based on two solutions on their neighbor solutions. Each plot is to study one retrained solution, and each point in the plot corresponds to one candidate solution from the neighbors of the retrained solution. We plot the increase in the error by applying post-training quantization of the solution using the base model parameters versus the decrease in the error by applying post-training on the retrained parameters. %In these plots the distance between the plotted solutions and the beacon is $\leq 6$.
%It is observed from the plots that almost all the points follow a linear relation between error increase before retraining and error decrease by using a neighbor retrained solution parameters.
%\begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\columnwidth]{images/beacon_1.png}
%    \caption{A plot for the error enhancement using one retrained model parameters (beacon). Each point corresponds to a neighbor solution to the retrained model solution. The x-axis corresponds to the increase in the baseline model error by evaluating solutions using baseli                                           nbne model parameters and the y-axis corresponds to the error degradation using the retrained parameters. }
%    \label{fig:beacon_1}
%\end{figure}

%This property is very beneficial in the search. We call the retrained solution a beacon. We can use retrained beacons instead of retraining all candidate solutions.

We defined an equation to compute the distance between candidate solutions to point out neighbor solutions. In our experiments, We found that the precision of the weights is more effective than the precision of the activations when finding neighbor solutions that can use the same retrained parameters. Thus, we only used the weights precisions in the distance computation. Also, we use the encoded values for the weights precision as defined in Section~\ref{sec:method-inference}. The distance between one solution and a beacon is defined as:
\begin{equation*}
 D_{ij} = \sum_{k=0}^{N} |s_{ik}-b_{jk}| ~~~,
\end{equation*}
where $D_{ij}$ is the distance between $solution_i$ and $beacon_j$. $N$ is the number of layers in the model. $s_{ik}$ is the precision of layer k weights in $solution_i$ and $b_{jk}$ is the precision of layer k weights in $beacon_j$.

Algorithm~\ref{alg:beacon} shows the steps for evaluating the error for a candidate solution using the beacon-based method. To save search time, we do not want to create beacons in unnecessary areas, such as areas where other objectives are not good. Thus, we define an area called beacon-feasible area as the area that beacons can be created in. All the search constraints constrain this area, but the error constraint in this area is higher than the search error constraint to allow high error solutions that would be feasible if retrained to be considered. In addition, it is possible to add more constraints to this area based on the designer's experience to decrease the number of created beacons such as thresholds for other objectives and not allowing low error solutions to be retrained. Low error solutions may not benefit much from retraining and can consume a lot of retraining time. If the solution is in the beacon-feasible area, we compute the distance between the solution and all existing beacons using the distance equation defined earlier. If the nearest beacon is farther than a predefined threshold, then this solution will be converted into a beacon by retraining the model using its variables. After retraining, the solution is added to the beacon list, and the nearest beacon is recomputed again. In this case, the nearest beacon is the solution itself, as it has been converted into a beacon by retraining. Finally, the error objective is re-evaluated using the nearest beacon model parameters.

\begin{algorithm}[H]
\SetAlgoLined
Evaluate error objective\;
Evaluate other objectives\;
 \If{solution is in beacon-feasible area}{
  Compute distance to all beacon\;
  \If{distance to nearest beacon > threshold}{
   Convert solution to a beacon by retraining the model using the solution variables\;
   Add beacon to beacons list\;
   Compute distance to all beacons;
   }
   Evaluate error objective using nearest beacon;
  }
 \
 \caption{Evaluate error for a candidate solution using beacon-based search.}
 \label{alg:beacon}
\end{algorithm}

==> files/method_tn.tex <==
\label{sec:method}
This section discusses the details of our proposed method for the Multi-Objective Hardware-Aware Quantization (MOHAQ) of the SRU-model for speech recognition. First, we explain how we apply the post-training quantization on the SRU. Next, we present the optimization algorithm used to select the layers' precisions guided by the hardware model. then, we explain how to enable retraining in a multi-objective search for setting mixed-precision quantization configurations. Finally, we discuss how we use the hardware models for guidance during the compression optimization.
\subsection{Post-training quantization of SRU model}
The Simple Recurrent Unit (SRU) was initially designed to overcome the parallelization difficulty in LSTM and other recurrent units. Outputs from the previous time-steps are used in the current time-step operations. This property makes it impossible to fully parallelize the M$\times$V operations over multiple time steps. In SRU, the outputs from the previous time-step are excluded from M$\times$V computations and only used in element-wise computations.

Another side effect for excluding the recurrent inputs from M$\times$V operations is that the number of weights used in the recurrent operations decreases significantly. Thus, it becomes possible to also exclude the recurrent part from low-precision quantization. We apply low-precision quantization on weights and activations used in M$\times$V operations only. Other weights are kept in a 16-bit fixed-point format. By doing so, We achieve our goal of reducing the model's overall size while keeping it performing with a low error rate. % Excluding the bias from quantization of LSTM has been done without significant effect on the model size~\cite{quantize-aji2020}.
%The last sentence here is somehow not linked to the context!-- Eren
We have both 16-bit fixed-point and integer precisions in the same model in different layers in our work.  We here explain how quantization has been applied to the weights and activations during inference and how we move from fixed-point to integer operations and the reverse.
\begin{itemize}
\item \textbf{Weights integer quantization with clipping:}
We applied integer linear quantization on the weight matrices. We used the Minimum Mean Square Error (MMSE) method to determine the clipping threshold~\cite{Sung_MMSE_2015}. We used the implementation for CNN quantization provided by OCS paper on github~\cite{postq-ocs-zhao19} as a base for our implementations. We then modified the implementation to work with SRU units and to support varying precision per layer. The range of the quantized values are [$-128$:127], [$-8$:7], and [$-2$:1] for 8-bit, 4-bit, and 2-bit, respectively.
\item \textbf{Weights 16-bit fixed-point quantization:}
It is used for the recurrent weights, bias vectors, and weight matrices that might be chosen to have 16-bit. Depending on the range of data, we compute the minimum number of bits required for the integer part. The rest of the 16-bits are used as a sign bit and the approximated fraction part.
\item \textbf{Activation integer quantization with clipping:}
Integer quantization of activations is similar to weights. However, since we cannot compute the range of vectors required for clipping threshold computation, we calculate the expected ranges. To compute expected ranges, we first use a portion of the validation data sequences. The predicted range of a given vector is calculated as the median value of the ranges recorded while running the validation sequences. In our experiments, 70 sequences were enough to compute the expected ranges.
\item \textbf{Activation re-quantization to 16-bit fixed-point:}
The activations are quantized to 16- bits the same way as the weights. If a vector is an output of an integer operation, we found it necessary to re-quantize the values into fixed points by dividing them by a scale value. The scale value is computed to return the vector range to the same range if quantization was not applied. The range of Non-quantized data is computed using a portion of the validation data sequences while using original model weights and activation, a.k.a, turning off quantization.
\end {itemize}

\subsection{Multi-objective quantization of neural network models}
\label{sec:method-inference}
During the compression/quantization of NN models, we have two types of objectives. The first one is the NN model performance metric, such as the accuracy or the error. The second type of objective is related to the efficiency of the hardware platform, such as memory size, speedup, energy consumption, and area. Treating the problem as a multi-objective problem provides the designer with various solutions with different options. The embedded system designer then can decide which solution is a trade-off suitable for the target application. We have used a Genetic Algorithm (GA) as it is one of the efficient multi-objective search optimizers. The multi-objective GA we used is called NSGA-II provided by the Pymoo python library~\cite{NSGA2-Deb-2002,pymoo}. 
%Our methods focus on speeding up the evaluations of candidate solutions during search to make it feasible. We select a GA that can fit the purpose of finding a good solution set within a reasonable time without claiming that this GA is the best for our search. 
As mentioned in Section~\ref{sec:back}, NSGA-II is a popular GA that supports more than one objective. NSGA-II showed the ability to find better convergence and better solutions spread near the actual Pareto-optimal front for many difficult test problems~\cite{NSGA-Srinivas-2000}. Thus, NGSA-II appears to be a good candidate for our experiments.

Most of the automated hardware-aware compression/quantization work uses a single objective and provides a single answer. The reason is that many compression methods require training or retraining to compensate for the accuracy loss caused by compression. The selection of the compression/quantization configuration is made iteratively during training epochs. Trying to turn the problem into a multi-objective problem would make it necessary to retrain all the evaluated solutions in the search space, and that would be infeasible. Our approach to tackle this problem relies on two observations. The first is that researchers are progressively enhancing post-training compression/quantization techniques. Thus, it is possible to evaluate candidate solutions by running inference only without any retraining. That is also useful for the case when the training data is not available. The second observation is that a retrained model using one candidate solution variables can be used as a retrained model for neighbor candidate solutions in the search space. We use this observation  in a method we call \textit{"beacon-based search"} (further explained in Section~\ref{sec:beacon}). So, if the inference-only search fails to find accuracy-wise accepted solutions, the beacon-based search can be applied. Nevertheless, if the designer wants, the beacon-based search can be applied from the beginning. The complete search framework is demonstrated in Figure~\ref{fig:idea}.
\begin{figure*}[h]
   \centering
   \includegraphics[width=1\columnwidth]{images/idea.png}
    \caption{Steps of the Multi-Objective Hardware-Aware Quantization (MOHAQ) method. The designer inputs the model pre-trained parameters, the hardware platform objectives equations, and any hardware constraints if they exist. Then the designer can apply inference-only search or beacon-based search. The beacon-based search is the search method that requires retraining of the model using some candidate solutions variables. The output of the search is a Pareto set of optimal solutions. Suppose the inference-only search resulted in solutions that had unaccepted accuracy levels. In that case, the designer can repeat the search using the beacon-based method.}
    \label{fig:idea}
\end{figure*}

Our problem is to select the precision for weights and activations per layer. A candidate solution has a number of variables that equals twice the number of layers. That is because each layer requires precision for the weight and precision for the activation. The possible precisions covered in this work are 2, 4, 8 bits integer, and 16-bit fixed point. We skipped precisions like 3, 5, and 6 because they are not frequently found in hardware platforms. However, the method is generic, and other precisions can be included. The candidate solutions variables are encoded into genetic algorithm representation. We use discrete values for the solutions variables that are 1, 2, 3, and 4. 2- bit is encoded into 1, 4-bit is encoded into 2, 8-bit is encoded into 3, and 16-bit is encoded into 4.
In addition to encoding and decoding, we select the number of generations, define fitness functions and constraints, then keep the library default configuration for the rest of GA steps such as the crossover, mutation, and selection. For each objective, we define a fitness function. All the objectives have to be either minimization or maximization objectives. Since Pymoo by default treats objectives as minimization objectives, we change the maximization objectives to be minimization objectives by negating them.


Initially, the search relies on post-training quantization (inference-only search). The evaluation of candidate solutions does not incorporate any training, and thus it is possible to carry out the search within a reasonable time. To evaluate one solution's error objective, we run the inference of the model and get the inference error value as the error objective that we want to minimize.
Another way to speed up the search is to define a feasibility area and if a solution falls outside this area, this solution is then directly excluded from the solution-pool and further search. We have used this to exclude solutions that have more than 8 percent points higher error rate compared to the baseline as such solutions were deemed irrelevant.



We use a subset from the validation data to evaluate a quantized model. We selected half of the validation data that would resemble the same distribution of speakers' gender and dialects in the testing dataset
%
%However, in our experiments, we have noticed that the gap between the validation error and the testing error varies significantly among the Pareto optimal solutions when we use the full validation set.
%To mitigate this variation (which can lead to solutions changing the order for the testing set compared to the validation set), we have split the validation set into smaller subsets (in this case, four subsets) and then taking the maximum error among the validation subset errors.
%This method has led to a better correspondence between validation errors and testing errors, and we will further explore and analyze it in the future.

% ToNo
It should also be noted that
the evaluations of candidate solutions in one generation are not related to the other candidate solutions.
Therefore, it is possible to parallelize the search over the candidate solutions and distribute the computation over multiple GPUs~\cite{Rezk-distGA-2014} with linear speedup.

\subsection{Beacon-based Search (Retraining-based Multi-objective Quantization) }
\label{sec:beacon}

So far, we have been focusing on using post-training quantization during the search for optimum quantization configuration to achieve a speedy evaluation of candidate solutions. However, at high compression ratios, we sometimes find that the post-training quantization is not achieving acceptable accuracy levels.
The accuracy can be improved by retraining the model using the quantized parameters. Still, as retraining is a very time-consuming process, it is infeasible to do for all candidate solutions. Therefore, we have developed a beacon-based approach that only retrains a small set of solutions, our beacons. Then we let other solutions share the retrained model (beacon) as a basis for their quantization instead of the original pretrained model.

To retrain the model, we used a Binary-connect approach \cite{lowp-binary-connect}, where quantized weights are used during the forward and backward propagation only, while full
precision weights are used for the parameters update step. Therefore, in the retrained model, we always have the floating-point parameters, which then can be used as a basis for various other quantization configurations. 

We have observed that if we retrained the model using one solution low precision configuration, the retrained parameters can be used with other low precision solutions and give a similar retraining effect. And thus we call a retrained model a beacon as it is used to predict retraining effect on many solutions. The next question is for which solutions a beacon (retrained model) is valid and for which solutions it is not valid. We have retrained the model for multiple low precision configurations (solutions) to generate multiple beacons. For each beacon we run a search that evaluate many solutions twice. Once using the baseline model parameters and once using the retrained model (beacon) parameters and computed the error decrease. The purpose if this experiment is to know the borders of the beacon validity. We found that if we successfully retrained a model on using a high error solution. The produced beacon is useful for most of the low precision solutions expect some solutions. However, the first layer, in some cases, would require special precision selection in the beacon. 

The exception solutions are solutions with extremely low precision in the first layer and solutions with the first layer fully in fixed-point precision. Those two cases needs special beacons crafted for them. The first layer is usually a high sensitive layer {add references}. Thus, having a very low precision in this layer needs to be fixed during retraining. However, retraining a solution with 2-bit precision in the first layer is a difficult task. The resulted beacon is not as good as the general beacon when applied to other solutions that does not have 2-bit in the first layer. Thus, we consider this a special case beacon and use it only for solutions that have 2-bit in the first layer. Also, using a beacon that has the first layer parameters adapted for integer precisions is not valid if the first layer weights and activations are in fixed-point. So, we create a special beacon for this case as well. 


We use Figures~\ref{fig:beacons} to visualize the effect of the beacons on different solutions. In Figure ~\ref{fig:beacons}a we use a model that has Four SRU-layers, three projection layers, and one FC connected layer. In Figure~\ref{fig:beacons}b, we use a model that has six SRU- layer, 5 projection layers, and one FC layer. In both figures, We plot the result of the experiment mentioned earlier, where we run a search that evaluates 400 solutions. The x-axis shows the increase in the error by a solution when quantizing the original model parameters compared to the non-quantized baseline error. The y-axis shows the decrease in error when quantizing the beacon model compared to the original quantized model. If the general beacon is used the solution is in the green color. If the solution has 2-bit weights in first layer, the solution is in red color. And, if the solution has fixed point weights and activations in the first layer, the solution is in blue color.	

To exemplify, we have marked one solution with a star in  Figure~\ref{fig:beacons}a. For this solution, the baseline model error rate is 17.2\%, and applying post-training quantization on this solution using the baseline model parameters gives an error rate of 22.2\%. Applying post-training quantization on the same solution using the beacon parameters gives an error rate of 18.7\%.	
Thus, we find the particular solution at 5 ($22.2-17.2$) on the x-axis and 3.5 ($22.2-18.7$) on the y-axis.	
%	
From the figure, we see a close to a linear relationship between the increase in the error using the baseline model parameters and the decrease in the error using the beacons parameters. We conclude that there is no need to retrain the model for all evaluated solutions during the search. It is sufficient to set up a small set of beacons to take the retraining accuracy increase into account during the search.	

\begin{figure*}[h]
   \centering
   \includegraphics[width=2\columnwidth]{images/beacons.png}
    \caption{Plots for the error enhancement using retrained model parameters (beacons). Each point corresponds to a solution. The x-axis corresponds to the increase in the baseline model error by evaluating solutions using baseline model parameters. The y-axis corresponds to the decrease in the error by evaluating solutions using beacon model parameters. Green solutions are using the general beacon. Red solutions are using the 2-bit weights first layer beacon. Yellow solutions are using the fixed point first layer beacon. }
    \label{fig:beacons}
\end{figure*}

We use the term beacon due to the similarity to its use in swarm robots search. Where the simple robots do not have the communication capabilities needed for the swarm to fulfill its task and some of the robots are assigned to be fixed communication beacons for the others~\cite{swarm-beacons-2013}. Similarly, when our search reaches an area were applying quantization on baseline model parameters lead to high error, a beacon is used to retrieve some of the accuracy loss. By the end, we get a solution-set that considers the retraining effect on the candidate solutions. Later on, when the designer selects a solution from the Pareto optimal set, the designer can use the beacon parameters directly or retrain the model using the selected solution parameters.


% ToNo: where to say this. And we need to align this to where we define these feasible areas
%

\subsection{Hardware-aware Optimization}

\input{files/hw-aware}
 

==> tables/bitfusion-6-beacon.tex <==
\begin{table}[!ht]
\centering
\caption{The beacon-based search Pareto-set of solutions resulted from applying NSGA-II  minimizing two objectives, $WER_V$ and speedup on the 6-SRU model. $WER_V$ is the error rate evaluated using the validation set. The speedup is computed using Bitfusion architecture model. The WER of the solutions when using the testing set is also previewed in the table ($WER_T$). $Cp_r$ is the compression ratio. $Base_F$ is the base model that can run on Bitfusion using a 16-bit full implementation.}
%\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.15cm}|p{0.75cm}|p{1.65cm}|}
\begin{tabular}{|c|c|c|c|c|}
\hline
Sol. & $WER_V$ & $Cp_r$&Speedup&
$WER_T$\\ \hline\hline

Base&13.9\% & 1x&-&16.1\% \\ \hline\hline
$Base_F$&13.9\% & 2x& 1x&16.1\% \\ \hline\hline

S1&	14.2\%&	10.3x&	16.0x&	16.9\% \\ \hline
S2&	14.4\%&	10.0x&	27.1x&	17.0\% \\ \hline
S3&	14.5\%&	10.5x&	34.6x&	17.2\% \\ \hline
%S4--S5 &--&--&--&--\\ \hline
S6&	14.8\%&	12.8x&	43.3x&	17.5\% \\ \hline
%S7--S8 &--&--&--&--\\ \hline
S9&	15.1\%&	13.1x&	48.9x&	18.2\% \\ \hline
%S10--s11 &--&--&--&--\\ \hline
S12&15.5\%&	12.0x&	50.3x&	18.0\% \\ \hline
%S13--S15 &--&--&--&--\\ \hline
S16&16.1\%&	13.5x&	52.6x&	18.6\% \\ \hline
\end{tabular}
\label{tab:bitfusion-beacon-6}%

\end{table}	



==> tables/bitfusion_beacon.tex <==
\begin{table}[!ht]
\centering
\caption{ The beacon-based search Pareto-set of solutions resulted from applying NSGA-II  minimizing two objectives, $WER_V$ and speedup on the 4-SRU model. $WER_V$ is the error rate evaluated using the validation set. The speedup is computed using Bitfusion architecture model. The WER of the solutions when using the testing set is also previewed in the table ($WER_T$). $Cp_r$ is the compression ratio. $Base_F$ is the base model that can run on Bitfusion using a 16-bit full implementation. Solutions start with $SI$ belongs to the inference-only search Pareto set and solutions start with $SB$ belongs to the beacon-based search.}
%\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.15cm}|p{0.75cm}|p{1.65cm}|}
\begin{tabular}{|c|c|c|c|c|}
\hline
Sol. & $WER_V$ & $Cp_r$&Speedup&
$WER_T$\\ \hline\hline

Base&14.9\% & 1x&-&17.2\% \\ \hline\hline
$Base_F$&14.9\% & 2x& 1x&17.2\% \\ \hline\hline

S1&	14.8\%&	11.8x&	20.2x&	17.5\% \\ \hline
S2&	14.9\%&	11.8x&	25.7x&	17.7\% \\ \hline
%S3--S4 &--&--&--&--\\ \hline
S5&	15.2\%&	11.8x&	32.1x&	18.2\% \\ \hline
%S6 &--&--&--&--\\ \hline
S7&	15.6\%&	13.3x&	37.3x&	18.8\% \\ \hline
%S8--S9 &--&--&--&--\\ \hline
S10&16.3\%&	14.5x&	42.3x&	18.5\% \\ \hline
%S11 &--&--&--&--\\ \hline
S12&16.7\%&	14.5x&	47.9x&	19.5\% \\ \hline
%S13 &--&--&--&--\\ \hline
S14&17.9\%&	15.6x&	48.8x&	20.3\% \\ \hline

\end{tabular}
\label{tab:bitfusion-beacon}%

\end{table}	



==> tables/lstm.tex <==
%\newcommand{\tabRNNLayer}{2.75cm}
%\begin{landscape}
\begin{table}[ht]
\centering
%\begin{threeparttable}
\caption{Number of operations and parameters in LSTM, SRU, and Bi-SRU. $m$ is input vector $x_t$ size, $n$ is the hidden vector $h_t$ size.}
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline \hline


Layer & \multicolumn{3}{c||}{$\#Operations$}&   \multicolumn{2}{c|}{$\#Parameters$} \\  \cline{2-6}


& MAC & E.wise & Nonlin. & Weights & Biases \\ 
\hline \hline

{LSTM} & $4 n^2 + 4 n m $& $8 n$ &
$5 n  $&
$4 n^2 + 4 n m $& $4 n$\\  \hline \hline

%\cline{2-6} 
%&$=LSTM_{mul}$&$             %=LSTM_{add}$&$=LSTM_{nonlinear}$&$=LSTM_{weights}$&$=LSTM_{biases}$ \\ \hline \hline

SRU &$3 n m $&$ 14 n$  &$2 n$&$3 n m + 2  n$ &$ 2 n$\\ 
\hline \hline

Bi-SRU &$6 n m$ & $28 n$  &$4 n$&$6 n m + 4  n$ &$ 4 n$\\ 
\hline \hline


\end{tabular}
\label{tab:complstm}%
%\begin{tablenotes}
%\item[]In the table we use the following symbols: $m$ is the size of input vector $x_t$, $n$ is the number of hidden cells in $h_t$,  
%\end{tablenotes}
%\end{threeparttable}
\end{table}	
%\end{landscape}





==> tables/model.tex <==
\begin{table*}[!ht]
\centering
\caption{The breakdown of the model used in the experiments. For each layer, we put the input vector size and the output vector size. Then, we compute the number of weights and operations for both MAC operations and other operations. We apply the formulas in Table ~\ref{tab:complstm}. Each layer is denoted as $L_x$, and each projection layer is denoted as $Pr_x$, where x is the layer index and FC is the fully connected layer.}
%\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.15cm}|p{0.75cm}|p{1.65cm}|}
\begin{tabular}{|c|c|c|c||c|c|c|c|c|c|}
\hline
&$L_0$ & $Pr_1$&$L_1$& $Pr_2$& $L_2$& $Pr_3$ &$L_3$& FC&Total \\ \hline\hline

Input vector size (m)&23&1100&256&1100&256&1100&256&1100&-	\\ \hline
Number of hidden cells (n) &550&256&550&256&550&256&550&1904&-	\\ \hline\hline
MAC operations &75900&281600&844800&281600&844800&281600&844800&2094400&5549500	\\ \hline
Element-wise operations &15400&-&15400&-&15400&-&15400&-&88000\\ \hline

Non-linear operations&2200&-&2200&-&2200&-&2200&1904&10704
\\ \hline\hline
Matrices weights &75900&281600&844800&281600&844800&281600&844800&2094400&5549500	\\ \hline
Vectors weights &4400&-&4400&-&4400&-&4400&-&17600	\\ \hline

\end{tabular}
\label{tab:model}%

\end{table*}	



==> tables/silago-old.tex <==
\begin{table*}[!ht]
\centering
\caption{ The Pareto-set of solutions resulted from applying NSGA2  minimizing three objectives, $PER_V$ and speedup and energy consumption. $PER_V$ is the error rate evaluated using the validation set. The speedup and energy consumption are computed using SiLago architecture model. The PER of the solutions when using the test set is also previewed in the table as $PER_T$. For each layer the numbers of bits used is written as W/A, where W is the number of bits for weights and A is the number of bits for activations. The base model is a 16-bit full implementation. The columns $\%Peak_S$ and $\%Peak_E$ show the percentage of peek speedup and peak energy saving achieved by each solution compared to the base solution. The peak performance in SiLago is reached by using 4-bit for all layers and activations.   }
%\begin{tabular}{|p{2cm}|p{1.5cm}|p{1.15cm}|p{0.75cm}|p{1.65cm}|}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Sol.&$layer_0$ & $Proj_1$&$Layer_1$& $Proj_2$& $Layer_2$& $Proj_3$ &$Layer_3$& FC & $PER_V$ & $Comp_r$& Speedup&  Energy $\textmu J$ &$\%Peak_S$&$\%Peak_E$&
$PER_T$\\ \hline\hline

Base&16/16 & 16/16 &16/16&16/16&16/16&16/16&16/16&16/16&16.2\% & 2x& 1x&16.4&-&-&17.2\% \\ \hline\hline

S1&8/8	&4/4	&4/4	&4/4	&16/16&	16/16	&8/8	&8	/8	&16.1\%&3.7x&	2.3x	&7.6	&57.6\%&	34.9\%&17.3\% \\ \hline

S2&16/16	&4/4	&4/4	&8/8&	4/4&	4/4	&8/8	&8/8&	16.2\%&	4.9x&	2.8x&	5.1&70\%&	51.6\%&	17.1\% \\ \hline

S3&8/8	&4/4	&4/4	&8/8	&4/4	&8/8	&4/4	&8/8&	16.3\%&	5.3x&	3x&	4.6&	75.4\%&	57.7\%&17.0\% \\ \hline

S4&8/8	&4/4	&4/4	&16/16&	4/4	&4/4	&4/4	&8/8	&16.4\%&	5.2x&	3x&	4.9&	76.6\%&	54.1\%&17.1\% \\ \hline

S5&8/8	&4/4	&4/4	&8/8	&4/4	&4/4	&4/4	&8/8	&16.6\%&	5.5x&	3.1x&	4.4&	77.9\%&	60.3\%&17.0\% \\ \hline

S6&8/8	&4/4	&4/4	&4/4	&4/4	&8/8	&4/4&	8/8	&16.6\%&	5.5x&	3.1x&	4.4&	77.9\%&60.3\%&17.5\% \\ \hline

S7&8/8	&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&8/8	&16.8\%&	5.7&	3.2x&	4.2&	80.4\%&63.2\%&17.4\% \\ \hline

S8&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&8/8	&17.3\%&	5.8x&	3.2x&	4.1&	81.1\%&64\%&
17.7\% \\ \hline

S9&8/8	&8/8	&4/4	&8/8	&4/4	&4/4&	4/4	&4/4	&18.5\%&	7.1x&	3.7x&	3.1&	94.2\%&	85.3\%
&19.3\% \\ \hline

S10&8/8	&4/4	&4/4	&8/8	&4/4	&4/4&	4/4	&4/4&	18.6\%&	7.5x&	
3.8x&	2.9&	96.8\%&	91.2\%&19.7\% \\ \hline

S11&16/16&	4/4	&4/4&	4/4	&4/4&	4/4&	4/4	&4/4	&18.9\%&	7.6x&	3.9x&	2.8&	99\%&	93.4\%&19.4\% \\ \hline

S12&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&4/4	&19.0\%&	8x&	3.9x&	2.6&	100\%&100\%&19.8\% \\ \hline


\end{tabular}
\label{tab:silago}%

\end{table*}	


